A fast platform for simulating flexible fiber suspensions applied to cell mechanics

We present a novel platform for the large-scale simulation of fibrous structures immersed in a Stokesian fluid and evolving under confinement or in free-space. One of the main motivations for this work is to study the dynamics of fiber assemblies within biological cells. For this, we also incorporate the key biophysical elements that determine the dynamics of these assemblies, which include the polymerization and depolymerization kinetics of fibers, their interactions with molecular motors and other objects, their flexibility, and hydrodynamic coupling. This work, to our knowledge, is the first technique to include many-body hydrodynamic interactions (HIs), and the resulting fluid flows, in cellular fiber assemblies. We use the non-local slender body theory to compute the fluid-structure interactions of the fibers and a second-kind boundary integral formulation for other rigid bodies and the confining boundary. A kernel-independent implementation of the fast multiple method is utilized for efficient evaluation of HIs. The deformation of the fibers is described by the nonlinear Euler--Bernoulli beam theory and their polymerization is modeled by the reparametrization of the dynamic equations in the appropriate non-Lagrangian frame. We use a pseudo-spectral representation of fiber positions and implicit HIs in the time-stepping to resolve large fiber deformations, and to allow time-steps not constrained by temporal stiffness or fiber-fiber interactions. The entire computational scheme is parallelized, which enables simulating assemblies of thousands of fibers. We use our method to investigate two important questions in the mechanics of cell division: (i) the effect of confinement on the hydrodynamic mobility of microtubule asters; and (ii) the dynamics of the positioning of mitotic spindle in complex cell geometries.

==> makefile <==
###
## generic makefile for latex projects
## Author: Abtin Rahimian
###

###
## Plain 'make' should work most of the time, other useful patterns are
##  $ make help              #to see this
##  $ make verb              #for debugging
##  $ make nobib             #for faster compilation
##  $ make PROJ=name         #for project with different name from the dir
##  $ make OUTEXT=dvi        #for dvi output with latex compiler
##
## to have a faster compilation, this does most of passes in quiet
## mode. The downside is that it hides the error in case of
## failure. To see the error either "make verb" or "make VERB='yes'".
###

## user flags
VERB	= yes
NOBIB   = no
PROJ	= method_main
LXX     = ${PDFLATEX}
OUTEXT  = pdf
SUMMARY = grep -in --color=always "\(error\|warn\|warning\|repeated\|skipping\)"
POSTSUM = awk '{ gsub("undefined", "\033[1;33m&\033[0m"); gsub("multiply defined", "\033[1;36m&\033[0m"); print }'
SYNC    = -synctex=1
ONEPASS = no

## programs
PDFLATEX = pdflatex
LATEX	 = latex
BIB	 = bibtex
DVI	 = dvipdf
PS	 = ps2pdf

## internal flag
QUIET	 =
LXFLAG 	 = -file-line-error -halt-on-error -shell-escape ${SYNC}
LXDFLAG  = ${LXFLAG}
BIBEXT   = bbl
INTEXT   = out

ifeq (${VERB},no)
  QUIET = -interaction=batchmode
endif

ifeq (${NOBIB},yes)
  BIBEXT = nobbl
endif

ifeq (${ONEPASS},no)
  LXFDFLAG += -draftmode
else
  INTEXT    = ${BIBEXT}
endif

TEXFILES = $(shell ls *.tex *.bib)

export

## project rules ##########################################################
###########################################################################
all: $(addsuffix .${OUTEXT}, ${PROJ})

## utility rules ##########################################################
###########################################################################
bib: $(addsuffix .${BIBEXT}, ${PROJ})

help:
	@head -18 ${MAKEFILE_LIST}

verb:   ## verbose make
	${MAKE} VERB=yes all

nobib:
	${MAKE} NOBIB=yes all

compress:
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4    	\
	-dPDFSETTINGS=/printer -dNOPAUSE -dQUIET -dBATCH   	\
	-dDownsampleColorImages=true			 	\
	-dDownsampleGrayImages=true 				\
	-dDownsampleMonoImages=true 				\
        -dColorImageResolution=400 				\
        -dGrayImageResolution=400 				\
        -dMonoImageResolution=400 				\
	-dColorImageDownsampleThreshold=1.5 			\
	-dGrayImageDownsampleThreshold=1.5 			\
	-dMonoImageDownsampleThreshold=1.5 			\
	-sOutputFile=${PROJ}-cmprs.pdf ${PROJ}.pdf

## generic rules ##########################################################
###########################################################################
%.pdf:${TEXFILES}
	${MAKE} LXX=${PDFLATEX} $*.${INTEXT}

%.dvi:${TEXFILES}
	${MAKE} LXX=${LATEX} $*.${INTEXT}

%.out:%.tex ${TEXFILES} %.${BIBEXT}
	${LXX} ${QUIET} ${LXDFLAG} $<
	${LXX} ${QUIET} ${LXFLAG} $<
	${SUMMARY} $*.log $*.blg | ${POSTSUM}
	${MAKE} clean

%.aux:%.tex ${TEXFILES}
	${LXX} ${QUIET} ${LXDFLAG} $<

%.${BIBEXT}:%.aux
	-${BIB} $* 1>/dev/null
	-${SUMMARY} $*.blg | ${POSTSUM}

%.nobbl:%.aux
	@echo "skipping the bib make step"

clean:
	${RM} *out *-blx.bib *run.xml *.nav *.snm *.toc *.cb *.cb2 *.spl *.cpt *.tdo *.lof *.lot *.auxlock figs/*.log figs/*.spl

cleaner:
	${MAKE} clean
	${RM} *log *blg $(addsuffix .aux, ${PROJ}) $(addsuffix .synctex.gz, ${PROJ})
	${RM} figs/*.dpth figs/*.md5 figs/*.dep
cleanest:
	${MAKE} cleaner
	${RM} $(addsuffix .pdf, ${PROJ}) $(addsuffix .dvi, ${PROJ}) $(addsuffix .${OUTEXT}, ${PROJ}) $(addsuffix .bbl, ${PROJ}) figs/external-*

.PHONY: clean cleaner cleanest
.SUFFIXES:
.SECONDARY:

